Incorporating Gradients to Rules: Towards Lightweight, Adaptive Provenance-based Intrusion Detection

As cyber attacks grow increasingly sophisticated and stealthy, it becomes more imperative and challenging to detect intrusion from normal behaviors. Through fine-grained causality analysis, provenance-based intrusion detection systems (PIDS) demonstrated a promising capacity to distinguish benign and malicious behaviors, attracting widespread attention from both industry and academia. Among diverse approaches, rule-based PIDS stands out due to its lightweight overhead, real-time capabilities, and explainability. However, existing rule-based systems suffer low detection accuracy, especially the high false alarms, due to the lack of fine-grained rules and environment-specific configurations. In this paper, we propose CAPTAIN, a rule-based PIDS capable of automatically adapting to diverse environments. Specifically, we propose three adaptive parameters to adjust the detection configuration with respect to nodes, edges, and alarm generation thresholds. We build a differentiable tag propagation framework and utilize the gradient descent algorithm to optimize these adaptive parameters based on the training data. We evaluate our system using data from DARPA Engagements and simulated environments. The evaluation results demonstrate that CAPTAIN enhances rule-based PIDS with learning capabilities, resulting in improved detection accuracy, reduced detection latency, lower runtime overhead, and more interpretable detection procedures and results compared to the state-of-the-art (SOTA) PIDS.

==> sections/General.tex <==
\subsection {Configurations in PIDS.} \label{sec:general}
Policies include variants and invariants. The invariants are signatures and rules generated from domain knowledge to match the potentially malicious behaviors and artifacts. The variants are weights associated with the signatures and rules, as well as the thresholds for determining the maliciousness. We systematically study the configurable components in provenance-based detection systems. 
Figure \ref{fig:principles_overview} shows an overview of our study on the existing provenance-based detection systems.
We divide the provenance-based detection into three stages: graph construction, feature extraction, and alarm generation, and summarize the existing methodologies in each stage. 
From our studies, we identify three common and configurable components among all provenance-based detection systems: node, edge, and threat assessment. 
We discuss how each component can be configured adaptively in this section.


\begin{figure}[h!]
    \centering
    \includegraphics[width=1.05\linewidth]{figures/overall_workflow.pdf}
    \caption{An overview of the workflow and techniques used in mainstream provenance-based detection systems and possible configuration options.}
    \label{fig:principles_overview}
    \vspace{-1.5em}
\end{figure}


\vspace{0.1in}
\noindent \textbf{Node Configuration}\label{node_configuration}
The node configuration determines the initial properties of nodes during provenance graph construction, which involves adding system events represented by two nodes connected by an edge. 
Many provenance-based detection systems tend to process all subjects and objects in events similarly. However, subjects are always processes and usually have comparable attributes, while objects could be quite different. We identify at least five categories of objects: processes, files, sockets, pipes, and memory objects. 
Each category participates in distinguishing system events and thus possesses unique characteristics. For instance, only sockets have source and destination IP addresses and ports. The differentiated categories and features allow the detection system to learn the fine-grained border of security baselines and thus enhance detection performance. For instance, if we know a certain range of IP addresses belong to the internal network, it is reasonable to assume that they are more likely to be associated with benign rather than malicious events. In our motivating example shown in Figure \ref{fig:attack graph}, the maliciousness associated with different IP addresses can improve its detection performance. In this case, \texttt{128.55.12.117} is a trusted internal IP address while \texttt{x.x.x.x} is an unknown external IP. Thus, the detection system should focus less on the activities of \texttt{128.55.12.117} but more on investigating the \texttt{x.x.x.x} related activities.

In summary, node configurations should be differentiated depending on node properties, independent of other nodes/edges. 
Adaptive node configurations can take various forms in provenance-based detection systems. In tag-based systems, it may involve a sophisticated node initialization policy. In anomaly-based systems, it could be an algorithm that assigns different weights to nodes when calculating anomaly scores. In graph matching-based systems, node differentiation may lead to using heterogeneous nodes in attack patterns.

\vspace{0.1in}
\noindent \textbf{Edge Configuration}
Edges in a provenance graph represent interactions between nodes. The edge information is usually used in the graph construction and feature extraction stages to change the malicious level of the nodes in the provenance graph. 
Each edge in the graph represents an event, which includes a subject, an object, and event-specific properties. However, many provenance-based detection systems only consider the event type, determining how to process an event without taking the subject and object into account. This coarse-grained approach limits detection capabilities, as the same event can have different implications between different subjects and objects. For example, writing to a socket can be part of an attack's exfiltration process, whereas writing to a local file does not necessarily disclose information. Moreover, an event with the same subject and object may have different implications in different environments, such as RDP connections being normal for personal hosts but not for some servers. In our motivating example in Figure \ref{fig:attack graph}, we expect the detection system to treat file write events differently. It is common when a process writes to a local \texttt{.txt} file. However, if the process writes to a file with an unusual \texttt{.tkn} suffix, this event should raise more concern.

% \begin{center}
% \fcolorbox{black}{gray!10}{\parbox{.96\linewidth}{
% \ZY{Principle 2: Known event? }
% }}
% \end{center}

In summary, edge configurations should be differentiated depending on the event information, including the subject, the object, and other event-specific properties.
Various provenance-based detection systems implement different methods to process the event information. In policy-based systems, it may involve a sophisticated propagation policy, while in anomaly-based systems, an algorithm may assign different weights to edges when calculating anomaly scores. Graph matching-based systems can introduce heterogeneous edges to attack patterns.

\vspace{0.1in}
\noindent \textbf{Threat Judgement Configuration}
During feature extraction and result generation stages, the detection systems need to determine the maliciousness of a system entity. 
The detection systems would gather all information from relevant nodes and edges to decide the detection results.
Many detection systems adopt a default set of criteria for all scenarios. However, these criteria should vary depending on the event's properties. 
In our motivating example shown in Figure \ref{fig:attack graph}, the attacker performed a typical download and execution kill chain. We expect detection systems to determine the maliciousness of a chain of behaviors accordingly in different environments. From the perspective of many detection systems, connecting from an external IP, downloading a file, executing it to write to \texttt{.tkn} files, and transferring those files out constitutes a series of suspicious actions. However, if such a chain of behaviors is the daily routine of the host, then it shouldn't raise significant concerns.

In summary, threat assessment configuration should be differentiated, taking all relevant nodes and edges into consideration. Different systems have different threat assessment methods. Tag-based systems aggregate tags on nodes, while anomaly-based systems may aggregate anomaly scores from individual components in the chain. Graph matching-based systems examine the alignment of the subgraphs.

\subsection{Adaptive Configuration in PIDS}
\label{exsiting_work_review}
We reviewed many main-stream PIDS proposed in recent years.
According to our investigation, all the existing adaptive configuration efforts fall in one of the three configurable components we identified.
% No matter how different their detection frameworks and customization methods are, they all followed at least one of the basic principles when configuring their detection systems.

\SLEUTH \cite{hossain2017sleuth} and \MORSE \cite{morse} are two similar tag-based APT detection and forensics systems.
While \SLEUTH didn't give any configuration adjustment methodologies for users, \MORSE can prune some edges to reduce the number of false alarms by setting two hyperparameters, \textit{tag attenuation} and \textit{tag decay}.
However, all hyperparameters in \MORSE should be set manually based on the domain knowledge and expertise.
Both \HOLMES~\cite{holmes} and \CONAN \cite{conan} can adjust the threshold to reduce the false alarms triggered by commonly seen benign activities on the hosts.

Theoretically, all learning-based detection systems can adaptively adjust their models based on the training data.
\small{ATLAS}\normalsize ~\cite{alsaheel2021atlas} extracts sequences from the graph and learns to classify them.
% used Long Short-term Memory (LSTM)~\cite{hochreiter1997long} network to classify the sequences.
% Although it did discriminate the nodes during the sequence extraction, it is hard to say they customized their systems because it mainly focused on malicious nodes.
While the system discriminates nodes during sequence extraction, it only focuses on malicious nodes, lacking the adaptation capability.
\WATSON~\cite{zeng2021watson} learns the node embedding and relative event importance from the benign traces, but it doesn't consider adjusting the alarm triggering function.

Anomaly-based systems can customize their benign models according to the training data from various environments.
% In our review of these works, we categorized their focuses during the customization process.
NoDoze \cite{nodoze} assigned an anomaly score to each edge in the provenance graph based on the frequency it appeared in the benign data and propagated the anomaly scores on the graph.
\PROVDETECTOR~\cite{wang2020you} extracts rare paths from the graph and embed them.
The path extraction and embedding lead to adaptive edge configuration.
The alarm decision can also be adaptive by adjusting the threshold.
\UNICORN \cite{han2020unicorn} embeds the extracted histograms from the provenance graph.
\SHADEWATCHER \cite{zengy2022shadewatcher} uses a recommendation model to detect the rare interactions in benign data.
Besides, it can automatically leverage expert feedback (mainly from false alarms) to refine its recommendation model.
% Anomaly-based detection systems, however, suffer from two main drawbacks.
% First, the detection results are difficult to interpret since the only information available about the detected attack is that it deviates from the benign behavior.
% Second, anomaly-based detection is vulnerable against mimicry attacks, where attacks pretend to be benign activities by repeating benign behaviors many times~\cite{goyalsometimes}.

Tab.~\ref{tab:survey_table} shows the results of our review.
To the best of our knowledge, this is the first and most comprehensive review of the adaptation design proposed in existing PIDS.
None of these systems proposes a method to adjust all three configurations.
Even though many works proposes configuration adjustment methods, most of them (except \SHADEWATCHER) do not incorporate a feedback mechanism to further improve the configurations and cannot adjust the configuration automatically.
% The most common problem of these customization designs is that they are incapable of dynamic adaptation, except \SHADEWATCHER.
% While all other detection frameworks, particularly anomaly-based detectors, can automatically adjust some configuration policies based on benign data, they cannot adjust their configurations after the training set has been fixed.
% In other words, customization relies on the training data and does not allow for dynamic adjustments based on the expert's feedback.
% Even if there might be a lot of false alarms, their configuration can not be adjusted automatically unless the training set is changed.


% Some of these detecting systems already have some designs about customized configurations.
% However, almost none of them does it automatically in a dynamic way.
% To show that, we designed and implemented an automatic configuration system to demonstrate this capability, based on tag-propagation-based APT detectors.
% Our system enables human-defined, blunt, and rigid detectors to adapt to any environment without compromising their detection capabilities.

\begin{table}[h!]\footnotesize
\centering
\begin{tabular}{cccc}
\hline
{\scriptsize Approaches} &
  \begin{tabular}[c]{@{}c@{}}{\scriptsize Node} \\ {\scriptsize Adaptation}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}{\scriptsize Edge} \\  {\scriptsize Adaptation}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}{\scriptsize Threat Judgement} \\ {\scriptsize Adaptation} \end{tabular} \\ \hline
SLEUTH \cite{hossain2017sleuth}       & \XSolidBrush & \XSolidBrush & \XSolidBrush  \\
CONAN \cite{conan}         & \XSolidBrush & \XSolidBrush & \Checkmark\\
HOLMES \cite{holmes}       & \XSolidBrush & \XSolidBrush & \Checkmark \\
POIROT \cite{poirot}       & \XSolidBrush & \XSolidBrush & \XSolidBrush \\
NODOZE \cite{nodoze}       & \XSolidBrush & \Checkmark & \XSolidBrush \\
PROVDETECTOR \cite{wang2020you}       & \XSolidBrush & \Checkmark & \Checkmark \\
MORSE \cite{morse}        & \XSolidBrush & \Checkmark & \XSolidBrush \\
UNICORN \cite{han2020unicorn}        & \XSolidBrush & \XSolidBrush & \Checkmark \\
WATSON \cite{zeng2021watson}        & \Checkmark & \Checkmark & \XSolidBrush \\
ATLAS \cite{alsaheel2021atlas}        & \Checkmark & \XSolidBrush & \Checkmark \\
SHADEWATCHER \cite{zengy2022shadewatcher} & \XSolidBrush & \XSolidBrush & \Checkmark \\ \hline
\end{tabular}
\caption{Adaptation design in existing PIDS. All of them (except \SHADEWATCHER) adapt their detection systems manually and statically.}
\label{tab:survey_table}
% \vspace{-1.5em}
\end{table}

==> sections/RelatedWork.tex <==
% Our work focus on solving the customized configuration problems on provenance-based APT detection system automatically.
\subsection{Provenance-based Intrusion Detection System}
PIDS detects system threats by analyzing information flow in the provenance graph.
A PIDS typically consists of three main phases: graph construction, feature extraction, and result generation, as illustrated in Figure \ref{fig:principles_overview}.
In the graph construction phase, the provenance data is converted to a provenance graph. 
While in the feature extraction phase, the detection system examines the provenance graph by various approaches~\cite{graph_embedding, graph_embedding2, goyal2018graph, hossain2017sleuth, morse, conan, nodoze, han2020unicorn, wang2020you} to extract crucial features. 
In the following result-generating phase, the extracted features are analyzed to determine the detection results.
% The ultimate goal of an APT detection system is to separate the malicious activities from the benign system activities.

Numerous PIDS have been proposed and improved to detect threats quickly and accurately. 
Most of them can be categorized into three classes: graph matching-based detection, learning-based detection, and tag-based detection\cite{li2021threat}.
Graph matching-based detection matches subgraphs with known malicious patterns to identify threats.
It usually involves graph embedding or other approximate algorithms for graph comparison. 
Learning-based detection learns the maliciousness of events based on statistical analyses of historical events in training and then applies the learned knowledge to detect threats.
Tag propagation-based detection abstracts the event history into tags and propagates tags to account for consequent interactions. Depending on the design of the detection framework, tags may contain different information, such as numbers denoting confidentiality and integrity~\cite{hossain2017sleuth, morse}, or a set of pre-defined behaviors~\cite{conan}. Eventually, the tags aggregate to a threshold and trigger alarms.
% Although the training does not affect the run-time overhead, anomaly detection still need to traverse sub-graphs to calculate the anomaly scores at run-time.

\noindent\textbf{Graph Matching-based Detection:}
RapSheet \cite{rapsheet} defines a set of rules to generate alerts for individual MITRE techniques and uses those alerts to construct a \textit{Tactical Provenance Graph (TPG)}. Then, threat scores are assigned to the TPGs to describe their "Likelihood of Attack" and "Typical Severity." Such threat scores are determined by relying on the online knowledge base.
Poirot \cite{poirot} establishes a knowledge base of attack behavior graphs and performs graph alignment to produce an alignment score. The alignment score is then compared with a threshold to determine whether an alert should be triggered. 
% Here the threshold represents the sensitivity of graph matching. Too high a threshold may lead to false negatives and too low a threshold may lead to false positives. The authors determine the threshold by trial and error.

\noindent\textbf{Tag Propagation-based Detection:}
\SLEUTH~\cite{hossain2017sleuth} presents a tag propagation-based method. It defines two different kinds of tags for every node: trustworthiness tags (t-tags) and confidentiality tags (c-tags), which are similar to the integrity and confidentiality tags in \MORSE. to make us concentrate on the important part of the provenance graph.
\HOLMES \cite{holmes}, published in 2019, constructs a high-level scenario graph (HSG) from the original provenance graph, then maps scenarios to the lifecycle of APT attacks and determines whether to generate alarms according to its policies. 
% Finally, a high-level scenario graph (HSG) is built after filtering out the noise and benign events from the original low-level graph. Given this very compact HSG, analysts can summarize and comprehend the overall process of entire attack.
% For every HSG, HOLMES evaluates a 7-tuple named as “threat tuple” because APT attacks have 7 major stages based on their understanding, which comes from “an extensive survey of APTs in the wild”.
% The element in this tuple is the coarse level indicating the dangerousness of each stage, such as “Low, Medium, High”.
% Finally, this very rough threat tuple is transferred into a threat score based on the domain experience.

\noindent\textbf{Learning-based Detection:}
\small{ATLAS}\normalsize ~\cite{alsaheel2021atlas} extracts sequences from the graph and uses Long Short-term Memory (LSTM)~\cite{hochreiter1997long} network to classify the sequences.
\UNICORN \cite{han2020unicorn} extracts histograms from the provenance graph and transfers them into numerical vectors using the HistoSketch \cite{yang2017histosketch} approach.
NoDoze \cite{nodoze} and its follow-up work \PROVDETECTOR \cite{provdetector}
are two SOTA works of anomaly detection on provenance data.
NoDoze traverses the provenance graph to a certain depth and calculates an anomaly score, while \PROVDETECTOR extracts rare paths from the graph and used the PV-DM model of doc2vec to embed them into numerical vectors before calculating the anomaly score.
Eventually, the anomaly score is compared with a manually defined threshold to determine whether an alert should be triggered. 
\SHADEWATCHER \cite{zengy2022shadewatcher} learns a recommendation model to rank the interactions by their likelihood of showing in benign scenarios.

There are several surveys on PIDS published in the last five years. Han et al. \cite{Han} published one of the first surveys on PIDS, but the survey only describes some opportunities and challenges without providing a systematic overview.
Li et al. \cite{apt_survey} came up with a general framework for PIDS, and Zipperle et al. \cite{zipperle} further expands on the taxonomy as well as the benchmark datasets. However, those works don't cover the approaches detection systems use to adjust the configuration adaptively.


\subsection{Adaptive Learning in Threat Detection}
In \S~\ref{exsiting_work_review}, We conduct a comprehensive survey on the adaptive design in recent PIDS work.
In addition, the idea of adaptive learning has been widely applied in the area of computer security, especially in malware detection systems.
In~\cite{blount2011adaptive}, Blount et. al present their work on proving an adaptive rule-based malware detection system to address the challenges due to the continuous evolution of malware.
They combine a rule-based detector with a evolutionary algorithm based on reinforcement learning.
Xu et. al. propose DroidEvolver, an adaptive malware detector can update itself given new data, in~\cite{xu2019droidevolver}.
Narayanan et. al. also uses online learning to adaptively update the detection model in~\cite{narayanan2016adaptive} and~\cite{narayanan2017context}.
In~\cite{chen2023continuous}, Chen et. al. fine-tune their detection model to adapt to new malware instances by active learning.
Their system can retrain the classifier using the specific labeled samples.

% \subsection{Machine learning applications on APT detection system}
% Xuan uses the Random Forest method on the network flow data to detect domains and IPs that are relevant to APT attacks \cite{do2021detecting}. 
% VulDeePecker generates embeddings from library/API function calls and then uses BLSTM neural network to do vulnerability detection \cite{vuldeepecker}. Xuan et al. uses neural networks (Graph Convolutional Network \cite{zhang2019graph} and Bi-directional LSTM \cite{graves2005bidirectional}) to detect and classify APT attacks based on the feature extracted from the network flow \cite{do2020apt}. Bodström et al. also focuses on detecting APT attacks by examining the network flow \cite{bodstrom2019novel}. They develop a multi-detection layer system where each layer has a separate neural network to take in the network flow data and output the detection results. Yan et al. uses an MLP network to classify DNS requests in the target network trying to locate the ones that are related to APT attacks \cite{yan2020discovering}. Niu et al. tries to address the difficulty of detecting fast evolving APT malware variants by using an LSTM neural network to capture time sequence features \cite{niu2022uncovering}. Deeptaskapt also uses LSTM to detect ATP attacks but on different type of datasets \cite{mamun2021deeptaskapt}. They apply the LSTM on log files of the system including information about files and processes. Wei et al. also uses LSTM with an attention mechanism to detect APT attacks from a different angle \cite{wei2021toward}. The data they use is a collection of system API calls. Xuan et al. aims to detect APT attack activities on the system \cite{do2022new}. They first build behavior profiles for processes in the system. Then, they use Graph Isomorphism Network (GIN) \cite{xu2018powerful} to take as input those profiles and decide if they are from APT malware or normal processes.  

% Tiresias trains recurrent neural network with security event sequences so that the neural network can predict the next event on the sequences. \cite{tiresias}

% FARE designs a clustering method with an input transformation network to better classifies low-quality labeled attack data to fine-grained categories. \cite{FARE}

% As listed above, most of state-of-the-art APT detection systems require manual configurations which involves numerous human effort, while others rely on some deterministic equations or knowledge bases to determine the configurations which leads to inconsistent performance in different environments. Recently, applying machine learning methods in the security field becomes increasingly prevailing. However, there haven't been a machine learning method proposed to solve the configuration problems in the APT detection systems. Our framework smoothly build machine learning module into the APT detection systems so that we can generate configurations not only automatically, but also adaptively.
